Randomized Nystr\"om Preconditioning

This paper introduces the Nystr\"om PCG algorithm for solving a symmetric positive-definite linear system. The algorithm applies the randomized Nystr\"om method to form a low-rank approximation of the matrix, which leads to an efficient preconditioner that can be deployed with the conjugate gradient algorithm. Theoretical analysis shows that preconditioned system has constant condition number as soon as the rank of the approximation is comparable with the number of effective degrees of freedom in the matrix. The paper also develops adaptive methods that provably achieve similar performance without knowledge of the effective dimension. Numerical tests show that Nystr\"om PCG can rapidly solve large linear systems that arise in data analysis problems, and it surpasses several competing methods from the literature.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage[utf8]{inputenc}
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{psfrag}
\usepackage{epstopdf}
\usepackage{bm}
%\usepackage{algorithm,algorithmic}
\usepackage[noend]{algpseudocode}
\usepackage{multirow}
\usepackage{array}
\usepackage{pbox}
\usepackage{array}
\usepackage{makecell}
\usepackage{siunitx}
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage{stmaryrd}
\usepackage{subcaption}
%\usepackage[colorinlistoftodos]{todonotes}
\usepackage{mathrsfs}
\usepackage[scr=boondox]{mathalfa}
\usepackage{xcolor}
\usepackage{makecell}
\definecolor{purple}{rgb}{0.3,0.0,.4}




\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

\newif\iftutorial
\tutorialfalse

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}
\newcommand{\R}[0]{\mathbb{R}}
\newcommand{\cN}[0]{\mathcal{N}}
\newcommand{\Hc}[0]{\mathcal{H}}
\newcommand{\normiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\jatnote}[1]{\textcolor{red}{\textbf{[JAT: #1]}}}
\newcommand{\mnote}[1]{\textcolor{purple}{\textbf{[MU: #1]}}}
\newcommand{\znote}[1]{\textcolor{blue}{\textbf{[ZF: #1]}}}
\def\P{{\mathbb{P}}} % probability measure
\def\E{{\mathbb{E}}} % expectation
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\tr}{\textrm{tr}}
\renewcommand\theadfont{\bfseries}

\sisetup{output-exponent-marker=\ensuremath{\mathrm{e}}}

\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}
\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\BREAK}{\STATE \algorithmicbreak}
\renewcommand{\Comment}[1]{%
\hfill \mbox{$\triangleright$\,#1}}
% algorithm storage macro
\algnewcommand\algorithmicstorage{\textbf{Storage:}}
\algnewcommand\Storage{\item[\algorithmicstorage]}
\newcommand{\fun}[1]{\texttt{#1}}
\algdef{SE}[SUBALG]{Indent}{EndIndent}{}{\algorithmicend\ }%
\algtext*{Indent}
\algtext*{EndIndent}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Nystr{\"o}m PCG}{Frangella, Tropp, and Udell}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Randomized Nystr{\"o}m Preconditioning\thanks{Submitted to the editors DATE.
\funding{ZF and MU were supported by
NSF Award IIS-1943131,
the ONR Young Investigator Program,
and the Alfred P. Sloan Foundation.
JAT was supported by ONR BRC Award N00014-18-1-2363 and NSF FRG Award 1952777.}}}

% Authors: full names plus addresses.
\author{Zachary Frangella\thanks{Center for Applied Mathematics, Cornell University, Ithaca, NY
  (\email{zjf4@cornell.edu}).}
\and Joel A.~Tropp\thanks{Department of Computing and Mathematical Sciences, California Institute of Technology, Pasadena, CA 91125-5000
  (\email{jtropp@cms.edu}).}
\and Madeleine Udell\thanks{Department of Operations Research and Information Engineering, Cornell University, Ithaca, NY(\email{udell@cornell.edu}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
%%% END HELPER CODE
%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:


%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:

